A coarse Erd\H{o}s-P\'{o}sa theorem

An induced packing of cycles in a graph is a set of vertex-disjoint cycles with no edges between them. We generalise the classic Erd\H{o}s-P\'osa theorem to induced packings of cycles. More specifically, we show that there exist functions $f(k,\ell)=\mathcal{O}(\ell k\log k)$ and $g(k)=\mathcal{O}(k\log k)$ such that for all integers $k\geq1$ and $\ell\geq3$, every graph $G$ contains either an induced packing of $k$ cycles of length at least $\ell$, not necessarily induced cycles, or sets $X_1$ and $X_2$ of vertices with $|X_1|\leq f(k,\ell)$ and $|X_2|\leq g(k)$ such that, after removing the closed neighbourhood of $X_1$ or the ball of radius $\ell$ around $X_2$, the resulting graph has no cycle of length at least $\ell$ in $G$. Our proof is constructive and yields a polynomial-time algorithm finding either the induced packing or the sets $X_1$ and $X_2$ when $\ell$ is a constant. Furthermore, we show that for every positive integer $d$, if a graph $G$ does not contain two cycles at distance more than $d$, then $G$ contains sets $X_1$ and $X_2$ of vertices with $|X_1|\leq12(d+1)$ and $|X_2|\leq12$ such that, after removing the ball of radius $2d$ around $X_1$ or the ball of radius $3d$ around $X_2$, the resulting graphs are forests. As a corollary, we prove that every graph with no $K_{1,t}$ induced subgraph and no induced packing of $k$ cycles of length at least $\ell$ has tree-independence number at most $\mathcal{O}(t\ell k\log k)$, and one can construct a corresponding tree-decomposition in polynomial time when $\ell$ is a constant. This resolves a special case of a conjecture of Dallard et al. (arXiv:2402.11222), and implies that on such graphs, many NP-hard problems, are solvable in polynomial time. On the other hand, we show that the class of all graphs with no $K_{1,3}$ induced subgraph and no two cycles at distance more than $2$ has unbounded tree-independence number.

==> _preamble/myBiblatex.tex <==

\usepackage[
    style=ieee,
    sorting=nyt,
    uniquename=init,
    defernumbers=true,
    maxnames=12,
    isbn=false,
    dashed=false,
    giveninits=false,
    datamodel=_preamble/mrnumber,
    citestyle=numeric-comp,
]{biblatex}


\RequirePackage{csquotes}
\RequirePackage{xpatch}
\RequirePackage{xstring}
\RequirePackage[fixed]{fontawesome5}

\newcommand{\linksymbol}{\scalebox{0.75}{\textcolor{black!75}{\faLink}}}


    \DeclareFieldFormat[article]{title}{``#1''}
    \DeclareFieldFormat[article]{volume}{\addnbspace\textbf{#1}}
    \DeclareFieldFormat[article]{number}{(#1)}
    \DeclareFieldFormat[article]{pages}{%
    \IfSubStr{#1}{Paper}{,\addnbspace#1}{:#1}}%
    
    \DeclareFieldFormat[article,book,incollection,inproceedings]{url}{%
        \linksymbol \href{#1}{#1}}
    \DeclareFieldFormat[article,book,incollection,inproceedings]{doi}{%
        \linksymbol \href{https://doi.org/#1}{DOI: #1}}
    \DeclareFieldFormat[article,book,incollection,inproceedings]{eprint:arxiv}{%
        \linksymbol \href{https://arxiv.org/abs/#1}{arXiv: #1}}
    \DeclareFieldFormat[article,book,incollection,inproceedings]{mrnumber}{%
        \linksymbol \href{http://www.ams.org/mathscinet-getitem?mr=#1}{MR: #1}}

    \DeclareBibliographyDriver{article}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/translator+others}}%
        \newunit
        \usebibmacro{title}%
        \newunit
        \printlist{language}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{bytranslator+others}%
        \newunit\newblock
        \printfield{version}%
        \newunit\newblock
        \usebibmacro{journal}%
        \printfield{volume}%
        \printfield{number}%
        \printfield{pages}%
        \newunit
        \usebibmacro{date}%
        \newunit
        \printfield{note}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
            {\usebibmacro{related:init}%
             \usebibmacro{related}}
            {}%
        \newunit\newblock
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}

    
    \DeclareBibliographyDriver{book}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/editor+others/translator+others}}%
        \setunit{\labelnamepunct}\newblock
        \usebibmacro{maintitle+title}%
        \usebibmacro{series+number(book)}%
        \printlist{language}%
        \newunit\newblock
        \printfield{edition}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{byeditor+others}%
        \newunit\newblock
        \printfield{volumes}%
        \newunit\newblock
        \setunit{\adddot\addspace}%
        \newblock
        \usebibmacro{publisher+location+date}%
        \newunit\newblock
        \usebibmacro{volume+part}%
        % \newunit
        % \usebibmacro{chapter+pages}%
        % \newunit
        % \printfield{pagetotal}%
        \newunit\newblock
        \printfield{note}%
        \newunit\newblock
        \iftoggle{bbx:isbn}
         {\printfield{isbn}}
         {}%
        % \newunit\newblock
        % \usebibmacro{doi+eprint+url}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
         {\usebibmacro{related:init}%
          \usebibmacro{related}}
         {}%
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}

        
    \DeclareBibliographyDriver{incollection}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/translator+others}}%
        \setunit{\labelnamepunct}\newblock
        \usebibmacro{title}%
        \newunit
        \printlist{language}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{in:}%
        \usebibmacro{maintitle+booktitle}%
        \newunit\newblock
        \usebibmacro{series+number}%
        \newunit\newblock
        \usebibmacro{byeditor+others}%
        \newunit\newblock
        \printfield{edition}%
        \newunit
        \iffieldundef{maintitle}
         {\printfield{volume}%
          \printfield{part}}
         {}%
        \newunit
        \printfield{volumes}%
        \newunit\newblock
        \printfield{note}%
        \newunit\newblock
        \usebibmacro{chapter+pages}%
        \newunit\newblock
        \usebibmacro{publisher+location+date}%
        \newunit\newblock
        \iftoggle{bbx:isbn}
         {\printfield{isbn}}
         {}%
        % \newunit\newblock
        % \usebibmacro{doi+eprint+url}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
         {\usebibmacro{related:init}%
          \usebibmacro{related}}
         {}%
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}

    \DeclareBibliographyDriver{inproceedings}{%
        \usebibmacro{bibindex}%
        \usebibmacro{begentry}%
        \textsc{\usebibmacro{author/translator+others}}%
        \setunit{\labelnamepunct}\newblock
        \usebibmacro{title}%
        \newunit
        \printlist{language}%
        \newunit\newblock
        \usebibmacro{byauthor}%
        \newunit\newblock
        \usebibmacro{maintitle+booktitle(inproceedings)}%
        \midsentence
        \newunit\newblock
        \usebibmacro{event+venue+date}%
        \newunit\newblock
        \usebibmacro{byeditor+others}%
        \newunit\newblock
        \printfield{volumes}%
        \newunit\newblock
        \usebibmacro{series+number}%
        \newunit\newblock
        \printfield{note}%
        \newunit\newblock
        \printlist{organization}%
        \newunit\newblock
        \usebibmacro{volume+part}%
        \newunit\newblock
        \usebibmacro{chapter+pages}%
        \newunit
        \usebibmacro{publisher+location+date}%
        \newunit\newblock
        \iftoggle{bbx:isbn}
         {\printfield{isbn}}
         {}%
        % \newunit\newblock
        % \usebibmacro{doi+eprint+url}%
        \newunit\newblock
        \usebibmacro{addendum+pubstate}%
        \setunit{\bibpagerefpunct}\newblock
        \usebibmacro{pageref}%
        \newunit\newblock
        \iftoggle{bbx:related}
        {\usebibmacro{related:init}%
          \usebibmacro{related}}
         {}%
        \usebibmacro{finentry}
        \iftoggle{linklinebreak}{\newline}{}
        \iffieldundef{url}{}{\printfield{url}\addspace}%
        \iffieldundef{doi}{}{\printfield{doi}\addspace}%
        \iffieldundef{eprint}{}{\usebibmacro{eprint}\addspace}%
        \iffieldundef{mrnumber}{}{\printfield{mrnumber}\addspace}}


\newtoggle{linklinebreak}
\AtEveryBibitem{%
    \iffieldundef{doi}{%
        \iffieldundef{url}{%
            \iffieldundef{eprint}{%
                \iffieldundef{mrnumber}{
                    \togglefalse{linklinebreak}%
                }{\toggletrue{linklinebreak}}
            }{\toggletrue{linklinebreak}}%
        }{\toggletrue{linklinebreak}}%
    }{\clearfield{url}\toggletrue{linklinebreak}}}

\renewcommand{\bibfont}{\scriptsize}
% \setlength{\bibitemsep}{1pt}
% \setlength{\bibhang}{2.5em}
% \xpretofieldformat{doi}
%   {\newline\linksymbol}
%   {}{}
% \xpretofieldformat{url}
%   {\newline\linksymbol}
%   {}{}
% \xpretofieldformat{eprint:arxiv}
%   {\iftoggle{linklinebreak}{\linksymbol}{\newline\linksymbol}}
%   {}{}
% \xpretofieldformat{mrnumber}
%   {\iftoggle{linklinebreak}{\linksymbol}{\newline\linksymbol}}
%   {}{}

\defbibheading{bibliography}{%
  \section*{References}%
}

%%% FOR ARXIV COMPILATION

\makeatletter
\let\blx@rerun@biber\relax
\makeatother
